Efficient D-optimal design of experiments for infinite-dimensional Bayesian linear inverse problems

We develop a computational framework for D-optimal experimental design for PDE-based Bayesian linear inverse problems with infinite-dimensional parameters. We follow a formulation of the experimental design problem that remains valid in the infinite-dimensional limit. The optimal design is obtained by solving an optimization problem that involves repeated evaluation of the log-determinant of high-dimensional operators along with their derivatives. Forming and manipulating these operators is computationally prohibitive for large-scale problems. Our methods exploit the low-rank structure in the inverse problem in three different ways, yielding efficient algorithms. Our main approach is to use randomized estimators for computing the D-optimal criterion, its derivative, as well as the Kullback--Leibler divergence from posterior to prior. Two other alternatives are proposed based on a low-rank approximation of the prior-preconditioned data misfit Hessian, and a fixed low-rank approximation of the prior-preconditioned forward operator. Detailed error analysis is provided for each of the methods, and their effectiveness is demonstrated on a model sensor placement problem for initial state reconstruction in a time-dependent advection-diffusion equation in two space dimensions.

==> alg.tex <==
The prior-preconditioned operator $\HMd$ is dense, and therefore, forming it
explicitly is prohibitively expensive for problem sizes of interest. Therefore,
we rely on randomized algorithms for estimating the objective function
$J(\vec{w})$ and its derivatives $\partial_j J(\vec{w})$.

The matrix $\HMd$ is Hermitian has rapidly decaying eigenvalues and is exactly
of rank $\min\{n,n_sn_t\}$. Therefore, we use the randomized estimator described in
Section~\ref{sec:randLA} to compute its log-determinant. Namely, letting $\mat{T}$ be the output of
of Algorithm~\ref{alg:randsvd}, applied to $\HMd$, we can approximate the objective function as 
\[
   \hat{J}(\vec{w}) \equiv  \logdet(\mat{I}+\mat{T}).
\]
To develop an randomized estimator for the derivative, we first simplify the
expression in~\eqref{e_partial_J2}. Write $\mat{I}_{n_t} = \sum_{k=1}^{n_t}
\vec{v}_k\vec{v}_k^*$, where vectors $\{\vec{v}_k\}_{k=1}^{n_t}$ form an
orthonormal basis for $\mathbb{C}^n$. By the linearity and cyclic property of
the trace operator, we can express $\partial_j J(\vec{w})$ as \[ \partial_j
J(\vec{w}) = \sum_{k=1}^{n_t} \trace\left( (\vec{v}_k \otimes \vec{e}_j)^*\FFp
(\mat{I} + \HMpd(\vec{w}))^{-1} \FFp^*(\vec{v}_k\otimes \vec{e}_j)\right)  =
\sum_{k=1}^{n_t}  \vec{f}_{jk}^* \mat{S} \mat{f}_{jk}, \] where $\vec{f}_{jk}
\equiv \FFp^*(\vec{v}_k\otimes \vec{e}_j)$ and $\mat{S} \equiv
(\mat{I}+\HMpd)^{-1}$. 

Let $\mat{T}_k$ denote the rank-$k$ truncation of $\mat{T}$ and let $\mat{T} = \mat{U}_T\widehat{\mat{\Lambda}}\mat{U}^*_T$ be its eigendecomposition. Then, we can approximate $\mat{S}$ using 
\begin{equation}\label{equ:Shat}
\widehat{\mat{S}} = (\mat{I} + \mat{U}_k\mat{\Lambda}_k\mat{U}_k)^{-1},
\end{equation}
where $\widehat{\mat{U}} = \mat{Q}\mat{U}_T$. Applying the Woodbury matrix identity
\[ \widehat{\mat{S}} \> =  \> \mat{I}- \widehat{\mat{U}}\mat{D} \widehat{\mat{U}}^* \] 
where $\mat{D} \equiv \text{diag} \left( \frac{\hat\lambda_i}{1 + \hat\lambda_i} \right) \in \mathbb{R}^{\ell\times \ell} $ and $\hat\lambda_i$ are the eigenvalues of $\mat{T}$.
This approximation can be used to estimate $\partial_j J(\vec{w})$. Write
\[\partial_j J(\vec{w}) \approx \sum_{k=1}^{n_t}  \vec{f}_{jk}^* \widehat{\mat{S}} \mat{f}_{jk} = \trace(\widehat{\mat{S}}\FFp^*\mat{E}_j\FFp). \]
 Observe that computing $\{\mat{f}_{jk}\}_{j=1,k=1}^{j=n_s,k=n_t}$ is expensive since it involves operations with the forward operator $\FF$ and the prior $\priorcov$; however, since it is independent of the vector $\vec{w}$, it can be precomputed.


We now summarize the computational cost of evaluating the objective function
and its derivative using the randomized estimators described above. The
objective function evaluation requires $(q+1)\ell$ matvecs involving the
transformed forward operator $\FFp$, $(q+1)\ell$ matvecs involving its adjoint
$\FFp^*$, and an additional $\mathcal{O}(k^2n)$ flops. For the derivative,
observe that  $\widehat{\mat{S}}\mat{f}_{jk}$ can be evaluated efficiently in
$\mathcal{O}(nk)$ flops, so that $\partial_j J(\vec{w})$ can be evaluated in an
additional $\mathcal{O}(knn_t)$ flops.

Next, we seek to quantify the error in randomized gradient computation. We begin by 
recording the following basic lemma:
\begin{lemma}\label{lem:basic}
Let $A$ be an $n \times n$ matrix and suppose $B$ is a symmetric positive
semidefinite matrix. Then, we have
\[
   |\trace(\mat{A}\mat{B})| \leq \norm{\mat{A}}_2\trace(\mat{B}).
\]
\end{lemma}
\begin{proof}
Let $\{ \vec{e}_j \}_{j = 1}^n$ be the (orthonormal) basis of eigenvectors of $\mat{B}$ and
let $\{ \lambda_j \}_{j = 1}^n$ be the corresponding (real, non-negative) eigenvalues.
\[
|\trace(\mat{A}\mat{B})| = |\sum_j \ip{\vec{e}_j}{\mat{A}\mat{B}\vec{e}_j}|
           \leq \sum_j \norm{\vec{e}_j}_2 \norm{\mat{A}}_2 \norm{\mat{B}\vec{e}_j}_2
           = \norm{\mat{A}}_2 \sum_j \lambda_j
           = \norm{\mat{A}}_2 \trace(\mat{B}).
\]
\end{proof}

We now present a result that quantifies the error in the gradient using the randomized approach. 
\begin{proposition}
 The error in the approximation to $\partial_j J(\vec{w}) $
\[ |\partial_j J(\vec{w})- \trace(\widehat{\mat{S}}\FFp^*\mat{E}_j\FFp)| \> \leq \> \| \FFp^*\mat{E}_j\FFp\|_2 |\trace(\HMd) - \trace(\mat{T})|. \]
\end{proposition}
\begin{proof}



As before, we denote $\mat{S} = (\mat{I}+\HMpd)^{-1}$, and use its approximation $\widehat{\mat{S}}$ as defined in~\eqref{equ:Shat}. 
We note,

\begin{equation}\label{e_inter1} 
|\partial_j J(\vec{w}) - \trace(\widehat{\mat{S}}\FFp^*\mat{E}_j\FFp)|= 
|\trace\left( (\widehat{\mat{S}}-\mat{S}) \FFp^*\mat{E}_j\FFp\right)| \leq 
\norm{\FFp^*\mat{E}_j\FFp}_2 \trace( \widehat{\mat{S}} - \mat{S}),
\end{equation}
where the inequality follows from Lemma~\ref{lem:basic}.
Focusing on $\trace(\widehat{\mat{S}} -\mat{S} )$, it is readily seen that
$\trace(\widehat{\mat{S}}) = \trace(\mat{I} + \widehat{\mat{\Lambda}})^{-1}$
and $\trace(\mat{S})  = \trace(\mat{I} + \mat{\Lambda})^{-1}$. This gives 
\begin{align*}
\trace(\widehat{\mat{S}} -\mat{S} ) = & \> \trace(\mat{I} + \widehat{\mat{\Lambda}})^{-1} - \trace(\mat{I} + \mat{\Lambda})^{-1} \\ 
=& \>\sum_{i=1}^\ell \frac{1}{1+\tilde\lambda_i} - \frac{1}{1+\lambda_i} + \sum_{i=\ell +1}^n 1 - \frac{1}{1+\lambda_i}\\
=& \>\sum_{i=1}^\ell \frac{\lambda_i - \tilde\lambda_i}{(1+\tilde\lambda_i)(1+\lambda_i)} + \sum_{i=\ell +1}^n \frac{\lambda_i}{1+\lambda_i}.
\end{align*}
With the following simple inequalities, using the fact that $\lambda_i,\tilde\lambda_i \geq 0$ 
\[  \frac{\lambda_i - \tilde\lambda_i}{(1+\tilde\lambda_i)(1+\lambda_i)} \leq \lambda_i -\tilde\lambda_i \qquad \frac{\lambda_i}{1+\lambda_i} \leq \lambda_i, \]
we have  
\begin{equation}\label{e_inter2}
 \trace(\widehat{\mat{S}} -\mat{S} ) \leq  \sum_{i=1}^n \lambda_i - \sum_{i=1}^\ell \tilde\lambda_i  = \trace(\HMd - \mat{T}).
\end{equation}
Combining~\eqref{e_inter2} with~\eqref{e_inter1} gives the desired result.
\end{proof}


==> theory.tex <==

The following might be needed. 

\begin{lemma}
Let $\hilb$ be a real separable Hilbert space. Suppose $A:\hilb\to\hilb$ is a
bounded linear operator and suppose $B:\hilb \to \hilb$ is a positive
selfadjoint trace class operator. Then, we have
\[
   \trace(AB) \leq \norm{A}\trace(B).
\] 
\begin{proof}
First note that since $A$ is bounded and $B$ is trace-class, then $AB$ is trace-class. Then,
let $\{ e_j \}_{j = 1}^\infty$ be the (orthonormal) basis of eigenvectors of $B$ and 
let $\{ \lambda_j \}_{j = 1}^\infty$ be the corresponding (real, non-negative) eigenvalues.
\[
\trace(AB) = \sum_j \ip{e_j}{ABe_j}
           \leq \sum_j \norm{e_j} \norm{A} \norm{Be_j} 
           = \norm{A} \sum_j \lambda_j 
           = \norm{A} \trace(B).
\]

\end{proof} 
\end{lemma}


==> tocdef.tex <==
% -----------------------------------------------------------
% hack to enable table of contents
% -----------------------------------------------------------
\makeatletter
\def\addcontentsline#1#2#3{%
  \addtocontents{#1}{\protect\contentsline{#2}{#3}{\thepage}}}
\long\def\addtocontents#1#2{%
  \protected@write\@auxout
    {\let\label\@gobble \let\index\@gobble \let\glossary\@gobble}%
    {\string\@writefile{#1}{#2}}}
\setcounter{tocdepth}{3}
\newcommand\tableofcontents{%
    \section*{%\contentsname\\[1ex]\noindent
        \@mkboth{\noindent%
           \MakeUppercase\contentsname}{\MakeUppercase\contentsname}}%
    \@starttoc{toc}%
    }
\newcommand*\l@section[2]{%
  \ifnum \c@tocdepth >\z@
    \addpenalty\@secpenalty
    \addvspace{1.0em \@plus\p@}%
    \setlength\@tempdima{1.5em}%
    \begingroup
      \parindent \z@ \rightskip \@pnumwidth
      \parfillskip -\@pnumwidth
      \leavevmode \bfseries
      \advance\leftskip\@tempdima
      \hskip -\leftskip
      #1\nobreak\hfil \nobreak\hb@xt@\@pnumwidth{\hss #2}\par
    \endgroup
  \fi}
\newcommand*\l@subsection{\@dottedtocline{2}{1.5em}{2.3em}}
\newcommand*\l@subsubsection{\@dottedtocline{3}{3.8em}{3.2em}}
\newcommand*\l@paragraph{\@dottedtocline{4}{7.0em}{4.1em}}
\newcommand*\l@subparagraph{\@dottedtocline{5}{10em}{5em}}
\makeatother
% --------------------- end hack


